The Coordinate Particle Filter - A novel Particle Filter for High Dimensional Systems

Parametric filters, such as the Extended Kalman Filter and the Unscented Kalman Filter, typically scale well with the dimensionality of the problem, but they are known to fail if the posterior state distribution cannot be closely approximated by a density of the assumed parametric form. For nonparametric filters, such as the Particle Filter, the converse holds. Such methods are able to approximate any posterior, but the computational requirements scale exponentially with the number of dimensions of the state space. In this paper, we present the Coordinate Particle Filter which alleviates this problem. We propose to compute the particle weights recursively, dimension by dimension. This allows us to explore one dimension at a time, and resample after each dimension if necessary. Experimental results on simulated as well as real data confirm that the proposed method has a substantial performance advantage over the Particle Filter in high-dimensional systems where not all dimensions are highly correlated. We demonstrate the benefits of the proposed method for the problem of multi-object and robotic manipulator tracking.

==> hidden_markov_explicit_noise.tex <==
% model_pca.tex
%
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}









\begin{tikzpicture}

  % Define nodes
  
  

    
   \node[latent]                               		(sta_pre) {$\sta_{\pre}$};
   \node[latent, right=of sta_pre]               		(sta_cur) {$\sta_{\cur}$};
   \node[latent, right=of sta_cur]               		(sta_nex) {$\sta_{\nex}$};
    
   \node[latent, below=of sta_pre]               	  	(pno_pre) {$\pno_{\pre}^d$};
   \node[latent, below=of sta_cur, right=of pno_pre]        	(pno_cur) {$\pno_{\cur}^d$};
   \node[latent, below=of sta_nex, right=of pno_cur]        	(pno_nex) {$\pno_{\nex}^d$};
    
   \node[obs, below=of pno_pre]                  		(obs_pre) {$\obs_{\pre}$};
   \node[obs, below=of pno_cur, right=of obs_pre]         	(obs_cur) {$\obs_{\cur}$};
   \node[obs, below=of pno_nex, right=of obs_cur]         	(obs_nex) {$\obs_{\nex}$};
    
    


%   \node[latent, above=of a_pre, xshift=-1.2cm] (w) {$\mathbf{w}$};
%   \node[latent, above=of a_pre, xshift=1.2cm]  (x) {$\mathbf{x}$};
%   \node[latent, right=2cm of a_pre]            (t) {$\tau$};
  
  


%   Connect the nodes
  \edge {sta_pre} {sta_cur} ; %
  \edge {sta_cur} {sta_nex} ; %
  
  \edge {pno_pre} {sta_pre}
  \edge {pno_cur} {sta_cur}
  \edge {pno_nex} {sta_nex}
  
  \edge {pno_pre} {obs_pre}
  \edge {pno_cur} {obs_cur}
  \edge {pno_nex} {obs_nex}
  
  \edge {sta_pre} {obs_cur}
  \edge {sta_cur} {obs_nex}

% 
  \plate {} {(pno_pre)} {$\forall d\in D$}
  \plate {} {(pno_cur)} {$\forall d\in D$}
  \plate {} {(pno_nex)} {$\forall d\in D$}

%   \plate {} {(w)(a_pre)(yx.north west)(yx.south west)} {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> noise_hidden_markov.tex <==
\begin{tikzpicture} 
   \node[latent]                      	  	(pno_pre) {$\pno_{\pre}$};
   \node[latent, right=of pno_pre]          	(pno_cur) {$\pno_{\cur}$};
   \node[latent, right=of pno_cur]          	(pno_nex) {$\pno_{\nex}$};
    
   \node[obs, below=of pno_pre]                  		(obs_pre) {$\obs_{\pre}$};
   \node[obs, below=of pno_cur, right=of obs_pre]         	(obs_cur) {$\obs_{\cur}$};
   \node[obs, below=of pno_nex, right=of obs_cur]         	(obs_nex) {$\obs_{\nex}$};

  \edge {pno_pre} {obs_pre};
  \edge {pno_pre} {obs_cur};
  \edge {pno_pre} {obs_nex};
  \edge {pno_cur} {obs_cur};
  \edge {pno_cur} {obs_nex};
  \edge {pno_nex} {obs_nex};
\end{tikzpicture}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=blue,inner sep=1pt,
minimum size=25pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent, fill=blue!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


